Analysing the potential of seq-to-seq models for incremental interpretation in task-oriented dialogue

We investigate how encoder-decoder models trained on a synthetic dataset of task-oriented dialogues process disfluencies, such as hesitations and self-corrections. We find that, contrary to earlier results, disfluencies have very little impact on the task success of seq-to-seq models with attention. Using visualisation and diagnostic classifiers, we analyse the representations that are incrementally built by the model, and discover that models develop little to no awareness of the structure of disfluencies. However, adding disfluencies to the data appears to help the model create clearer representations overall, as evidenced by the attention patterns the different models exhibit.

==> disfluencies.tex <==
\section{Disfluencies}

%RAQ: This is just a draft. Some of the points here may end up in the Introduction or a Related Work section

In this section we write an overview of the linguistic theories of disfluencies, what exactly we stress more or less will depend on the tests we describe in the rest of the paper.

In spontaneous spoken language, utterances contain disfluencies. 

\paragraph{Disfluency rates.}
Disfluencies occur at the rate of about six per 100 words in task-oriented conversation \cite{bortfeld2001disfluency}.
They increase when speakers face heavier planning demands (e.g., unfamiliar domain, longer turns).
Rates of disfluencies differ in speech to human partners versus artificial partners: disfluencies, in particular filled pauses (hesitations such as {\em uh, uhm}) are more frequent in human-human conversation \cite{oviatt1995predicting,shriberg1996disfluencies}. \newcite{shriberg1996disfluencies} suggests this may be due to the special role of fillers, which may help people coordinate conversational exchanges. 


\paragraph{Form of disfluencies.}
The vast majority of reparanda are between 1 and 3 words long. For example, \newcite{Hough15Thesis} reports a mean length of 2.068 words (sd=1.428) for substitutions (i.e., repairs) in the Switchboard corpus \cite[Table 4.8 and Fig.~4.2 in pages 122-123]{Hough15Thesis}. 


Editing expressions (e.g., \emph{I mean, rather, that is, sorry, oops}) are rare.
% --- due to their low numbers, they are not even included in the counts by \cite{bortfeld2001disfluency}. 
\newcite{Hough15Thesis} finds that only 18.52\% of substitutions in the Switchboard corpus contain an explicit editing term.


\paragraph{How disfluencies are processed.}

The processing of disfluencies has been investigated both in NLP and Psycholinguistics. 
In NLP, the traditional approach to processing disfluencies has been to filter them out before or during parsing, prior to any process of semantic interpretation \cite{stolcke1996statistical,heeman1999speech,charniak2001edit}. While this ``filtering'' approach may have practical advantages, it is incompatible with the large body of psycholinguistic evidence regarding the immediacy of interpretation during language comprehension \cite{altmann1999incremental} [ADD MORE REFS]. Work on psycholinguistics has therefore focused on  investigating how the human comprehension system processes disfluencies as part of the task of building interpretations incrementally \cite{levelt1989speaking,FerreiraEtal2004}.




% Mention that more recent approaches to disfluencies in computational linguistics are not based on filtering, but rather take into account incrementality. And exploit disfluencies in language understanding and generation. 



Main empirical facts about how humans process disfluencies:

\begin{enumerate}

\item The comprehender faces what \newcite{levelt1983monitoring} calls the \emph{continuation problem}: the need to identify the (beginning and end of the) reparandum and the repair onset. Evidence shows that there are no clues (prosodic or otherwise) present during the reparandum. Thus the identification of the disfluency takes place at or after the moment of interruption (typically during the repair). Here there may be prosodic changes, but such clues are usually absent \cite{levelt1983prosodic}. 
\newcite{FerreiraEtal2004} point out that ``the language comprehension system is able to identify a disfluency, likely through the use of a combination of cues (in some manner that is as yet not understood)''.

\item People have less trouble understanding utterances with filled pauses and repeats than those with corrective repairs \cite{tree1995effects}.

\item Disfluencies, in particular repairs, involve some form of reanalysis. In this sense, there are parallelisms with the processing of garden-path sentences: the parser may pursue an incorrect syntactic analysis, which leads to revision (e.g., \emph{The girl selected for the role celebrated with her parents} -- it is common to first analyse this sentence with ``the girl'' as the active subject of ``selected'', and only later realise that this is a passive construction). 

\item Certain structural features make the reanalysis process more difficult. For example, the longer the parser has been committed to the wrong analysis, the more trouble it has recovering the right one \cite{ferreira1991recovery,bailey2003disfluencies}. In the case of disfluencies, this means that the longer the reparandum, the more difficult the processing (see comments above of reported mean length of reparanda). 

\item Certain structural features make the reanalysis process easier. For example, if the ``wrong'' word to be corrected is only partially articulated (i.e., it is truncated), or if there is an explicit editing term  (such as a filled pause) followed by a correction, the disfluency is easier to handle cite{brennan2001listeners}.

\item Information associated with the reparandum is only partially deactivated by the reanalysis process \cite{FerreiraEtal2004}. For example, a disfluency can make a garden-path sentence easier to understand. A sentence such as \emph{``The girl chosen -- uh selected for the role celebrated with her parents''} is easier to understand than the same sentence with no disfluency or with a reparandum verb such as \emph{picked} -- \emph{``The girl picked selected for the role celebrated with her parents''}. The idea is that \emph{chosen} activates the correct passive structure for the sentence and that structure lingers for the remainder of the utterance making it easier to understand than with \emph{picked}.


\end{enumerate} 




%``disfluencies are part and parcel of grammatical systems of natural languages'' \cite{ginzburg-fernandez-schlangen:2014:disfluencies}, where `grammar' is taken to be ``a mechanism that enables us to characterize the coherently interpretable conversational events''.





==> results.tex <==
\section{Testing Seq2Seq }

\begin{table*}\centering
\begin{tabular}{|l@{\ }c@{\ }l||cc|cc||c|}\hline
 		& & & \multicolumn{2}{c|}{\bf seq2seq} &  \multicolumn{2}{c||}{\bf attentive seq2seq} & MemN2N \\\hline
 \multicolumn{3}{|c||}{train / test}      & all sequences & API calls & all sequences & API calls & API calls \\\hline
bAbI   & /  & bAbI     & 83.2 (94.4) & 0.00 (59.8) &  100 (100)  &   100 (100) & 100\\ 
bAbI+ & /  & bAbI+   & 89.4 (97.0) & 0.06 (67.9) & 100 (100)   & 99.8 (99.9) & 53 \\
bAbI   & /  & bAbI+   & 66.0 (75.2) & 0.00 (55.2) & 88.1 (92.5) & 50.8 (90.2) & 28 \\
bAbI+ & /  & bAbI     & 84.2 (95.7) & 0.06 (69.1) & 100(100)    &  100(100)      & 99 \\ \hline
\end{tabular}
\caption{Sequence accuracy (word accuracy in brackets) on the test set for all generated system responses and API calls only. The last column shows accuracy on the test for the retrieval-based MemN2N system, as reported by \newcite{shalyminov2017challenging} .}
\label{tab:results}
\end{table*}

\begin{table*}\centering
\begin{tabular}{|l@{\ }c@{\ }l||cc|cc||c|}\hline
 		& & & \multicolumn{2}{c|}{\bf seq2seq} &  \multicolumn{2}{c||}{\bf attentive seq2seq} & MemN2N \\\hline
 \multicolumn{3}{|c||}{train / test}      & utterances & API calls & utterances & API calls & API calls \\\hline
bAbI   & /  & bAbI     &  100(100)  & 0.00 (59.8) &  100 (100)  &   100 (100) & 100\\ 
bAbI+ & /  & bAbI+   &  100(100) & 0.06 (67.9) & 100 (100)   & 99.8 (99.9) & 53 \\
bAbI   & /  & bAbI+   & 82.4 (84.6)  & 0.00 (55.2) & 88.1 (92.5)  & 50.8 (90.2) & 28 \\
bAbI+ & /  & bAbI     &  100(100) & 0.06 (69.1) & 100(100)    &  100(100)       & 99 \\ \hline
\end{tabular}
\caption{Sequence accuracy (word accuracy in brackets) on the test set for utterances (non-API-call responses) and API calls only. The last column shows accuracy on the test for the retrieval-based MemN2N system, as reported by \newcite{shalyminov2017challenging} .}
%\label{tab:results}
\end{table*}

Our results, which can be found in Table \ref{tab:results}, indicate that an encoder-decoder model with attention can achieve a high accuracy on both the bAbI and bAbI+ data, whereas a model without attention cannot.
These results confirm that models trained on data without disfluencies struggle when these are introduced at testing time: although the overall accuracy of the dialogue is still high (93\% of the sequences are correct), the API call accuracy falls back to little over 50\%.

Models trained on data containing disfluencies directly, however, show near-perfect generalisation to test data containing disfluencies, a result that stands in stark contrast with the findings of \citet{eshghi2017bootstrapping} and \citet{shalyminov2017challenging}.
\textcolor{red}{This discrepancy gives rise to several questions concerning the inner workings of these models, which we will address in the next section. Be more specific?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  Other tables to have a full overview of all numbers etc. 
%%  If you need any others let me(Sanne) know.

%\begin{table}[ht!]
%\begin{tabular}{|l|c|c|}
%\hline
%trained on:   & bAbI         & bAbI+ \\ \hline
%full dialog   & 88.1 (92.5)  &  100 (100)   \\
%api-calls     & 50.8 (90.2)  &  99.8 (99.9) \\
%not api-calls & 92.8 (92.8)  &  100 (100)   \\\hline
%\end{tabular}
%\caption{Word and sequence accuracies for different components of the data on bAbI+ data, word accuracy in brackets}
%\label{tab:errorsplit}
%\end{table}

%\begin{table}
%\centering
%\begin{tabular}{|l|c|c|} \hline
%train/test & all sequences & API-call only \\ \hline
%babi/babi   & 83.2(94.4) & 0.0(59.8) \\ 
%babi+/babi+ & 89.4(97.0) & 0.06(67.9) \\
%babi/babi+  & 66.0(75.2) & 0.0(55.2) \\
%babi+/babi & 84.2(95.7) & 0.06(69.1) \\ \hline
%\end{tabular}
%\caption{Sequence and word accuracy (within brackets) for different models trained without attention}
%\label{tab:noatt}
%\end{table}


==> task.tex <==
\section{bAbI data}

%In this section, we introduce the babi task and the babi+ task, and report on our results (accuracies) using a seq2seq model. 

%%% General introduction
The bAbI dialog tasks were originally designed as a prerequisit for end-end goal-oriented dialog systems \cite{bordes2016learning}. 
%They are introduced by FAIR %TODO: add reference?
%as an extension of the Visual Question Answering tasks
%, a task that also relies on a models ability to extract the semantic core of language.
The dialogs represent human-bot interactions within the restaurant domain, where the end-to-end system is trained to utter the correct bot utterances including API-calls that reflect what restaurant reservation is to be made.
\red{Justify why is it small etc. because models should learn with small data}

%%% Introduction of different tasks 
There are six distinct tasks, five tasks created from simulation that increase in complexity per task and a sixth task that is adapted from existing data.
In simulation, user queries are created by sampling an entry for 
each field type: Cuisine; location; party size; price range.
Each task represents a different aspect of dialog: Predicting an API-call; Updating an API-call; 
Displaying options; Providing extra information; and conducting full dialog. 
%An example of dialog for task 1-5 is displayed in Figure \ref{fig:bAbIdata}. 

%\begin{figure}[ht!]
%\centering
%\includegraphics[width=.5\textwidth]{images/babi-tasks}
%\caption{Different tasks \cite{bordes2016learning}}
%\label{fig:bAbIdata}
%\end{figure}

%The 6th bAbI task is adapted from dialogs used for the Dialog State Tracking Competition (DSTC2). %TODO: add reference
%States are used to generate API-calls and dialogs are shaped in the same format as other tasks.
%Introduce shortcomings of bAbI 
%There are a lot of errors in the data for task 6 due to speech recognition errors and mistakes made by both the bot and the humans. 

%%% Something about babi+
%Due to the fact that bAbI data for task 1-5 is generated from simulation, it is very artificial. 
%The jump from completely artificial dialogs to task 6 is quite big, several aspects which are present in natural language are missing in the bAbI dialogs of task 1-5.
%Add a sentene?
Eshgi et al. \cite{eshghi2017bootstrapping} noted that even though there is increase in goal-complexity, there is no increase in incremental lexical complexity which is integral to
natural language. 
To mitigate this they introduced bAbI+, an extension of the first bAbI task with everyday%What does it mean, everyday 
incremental dialogue phenomena. 
They focused on disfluencies and added hesitations, restarts, and corrections to the dialogs through fixed patterns for a given percentage of utterances. 
%They introduced these correction to the first task, as a different type of complexity to increase. 
%The first task is to correctly predict api-calls. 

%%% Show dislfuencies examples:
Disfluences are added through patterns which operate on words or partial phrases. The procedure is the same as Shalyminov et al. and source code 
is available in their paper \cite{shalyminov2017challenging}\\ 
Correction are added on slot-values and are of the type: \textit{[incorrect value] sorry [correct value]}. 
Different words are used in place of sorry, known in literature as "editing term". 
The value is not limited to a single word, for example "in london" or "in an expensive price range".\\
%TODO: check if these phrases really exist in data
Hesitations are added in place of a single word: \textit{[token] uhh [continuation]}\\
Restarts are introduced in place of a word or small sentence: \textit{[token] uhm yeah [utterance from beginning]} Again, different words are used in place of "uhm yeah". 

\red{Some sort of headings?}
%%% Introduce some baselines on bAbI
Bordes et al. present several baselines on the six bAbI tasks: 
Rule based models, classical information retrieval models (TF-IDF, nearest neighbour), supervised embedding models, 
and neural models(memory networks with and without match type).
%Models perform relatively well on the first 5 tasks, however result drop drastically when moving over to task 6, which is adapted from actual spoken dialogs with actual bots.
%TODO: add results?? 

%%% Introduce some baselines on babi+ and explain formal grammar thing. 
For the bAbI+ task memory networks were tested as well as a formal grammar based system. 
They find that even when trained on data with disfluencies, the memory network does get an accuracy of more than 50\%.
They overcome this by introducing a formal grammar which parses the disfluencies through grammatical knowledge constructed manually.

%%% introduce seq2seq
\section{Experimental Setup}
\subsection{Model}

Memory networks are harder to diagnose and more complex in nature. 
It is unclear if the bAbI tasks really require an external memory unit. %Figure out how memory networks really work.
Instead a sequence to sequence was trained for the tasks.  
Both the encoder and the Decoder are LSTM units with one layer.

The input sequence includes the memory of the rest of the dialog. %This was probably done before, reference this
In practice this means that for in dialog line i the data is transformed as follows:
$$ in_i = in_1 + out_1 + in_2 + out_2 + ... + in_i$$
$$ out_i = out_i $$


To help with the task and help with analysing afterwards attention mechanism was used. %REference attention
%REference machine?
Dropout was used, a percentage of 0.2 for both encoder and decoder. %also explain why it is sensible
%Reference dropout
The settings for hyper parameters are shown in table \ref{tab:hyperparam}

\begin{table}[ht!]
\centering
\caption{Table with hyperparameters}
\label{tab:hyperparam}
\begin{tabular}{|l|c|} \hline
 %& \\ \hline
 Hidden layer size & 500 \\ \hline
 Embedding size & 128 \\ \hline
 Batch size & 32  \\ \hline
 learning rate  & 0.001 \\ \hline
%src_vocab=50000
trained for x epochs  & 20 \\ \hline
\end{tabular}
\end{table}

The optimal value for the hidden layer was determined empirically, 
experiments were run for each deviation of 100 nodes (100,200,300,400,500,600). 
For both bAbI and bAbI plus task, A network with hidden layers sized 500 performed best.
%NOTE: encoder en decoder different size hidden layer??


\subsection{Setup}
%\subsubsection{Preprocessing/Experimental setup (title? placing?)}
%Something on how the model gets the data/ preprocessing
For each task 1000 training dialogs, 1000 development dialogs and 1000 test dialogs are available. For task 1-5 an additional test set is available with out of vocabulary instances, also consisting of a 1000 dialogs. 
Whenever the bot speaks twice, this is denoted in the data as “\textless SILENCE\textgreater”. 

%TODO: dit duidelijker maken?? met het plaatje?
%TODO: of the input sequence dinges hier?

Two sets of models were trained, one with attention and one without.
For each set, two models were trained, one on bAbI task 1 data and one on bAbI+ data. 
All models are evaluated on their matching and the opposing dataset, resulting in a total of eight experiments.

For each experiment data was fed in line by line and both word accuracy and sequence accuracy are reported.
Besides the word and sequence accuracy of each sequence in the dialog including the API-call, 
word and sequence accuracy of just sequences that are API-calls are reported for models without attention


\section{Results}

%Models were evaluated for babi/babi babi/babi+ babi+/babi+ babi+/babi. 
In Table \ref{tab:lemon-copy} the results are shown with attention and in Table \ref{tab:noatt}. 


\begin{table}
\caption{Table for training without attention for both all sequences and only API-calls. Values shown are sequence accuracy in percentages correct. and the values in brackets are word accuracy.}
%TODO: make caption shorter
\label{tab:noatt}
\begin{tabular}{|l|c|c|} \hline
train/test & all sequences & API-call only \\ \hline
babi/babi   & 83.2(94.4) & 0.0(59.8) \\ 
babi+/babi+ & 89.4(97.0) & 0.06(67.9) \\
babi/babi+  & 66.0(75.2) & 0.0(55.2) \\
babi+/babi & 84.2(95.7) & 0.06(69.1) \\ \hline
\end{tabular}
\end{table}

\begin{table}[ht!]
\centering
\caption{Sequence accuracy and word accuracy in brackets on task 1 for all sequences, all models are trained with attention}
\label{tab:lemon-copy}
\begin{tabular}{|l|c|c|}
\hline
train / test & all sequences\\ \hline  \hline
bAbI/bAbI   & 100 \\ \hline
bAbI+/bAbI+   & 99.8  \\ \hline
bAbI/bAbI+   & 88.1  \\ \hline
bAbI+/bAbI    & 100  \\ \hline
\end{tabular}
\end{table}

Both the results for bAbI to bAbI and bAbI+ to bAbI+ are high, as expected. 
This shows that a sequence to sequence model can learn both tasks well. 
The results on bAbI to bAbI+ show that indeed disfluencies pose a problem for the model.
The results of bAbI+ to bAbI show that generalising is not a problem in itself, 
generalising to the simpler task happens without fail. 



%Two questions arise that we try to answer with analysis in the following section. 
%Why can't the bAbI trained model do the bAbI+ data and what are the mistakes that are made?
%How is the model that learned to do the bAbI+ task perform the task and is it consistent with the theory introduced in the background section of this paper?
\red{Skip heading? Can we make this comparison?}

\subsection{Comparing to Memory Networks}
Similar to Shalyminov et al. we have 4 test setup's. \cite{shalyminov2017challenging}
They reported sequence accuracy for same-dataset evaluation and cross-dataset evaluation of Memory networks. 
Their results are shown in table \ref{tab:lemon}.
Similar scores for the Seq2Seq model are shown in table \ref{tab:lemon-copy}
These surprising results indicate sequence to sequence models, with at least 500 hidden nodes, are complex enough for these tasks. 
%Which models does the task better is indiscernible since both perform at ceiling level.

\begin{table}[ht!]
\caption{MemN2N API-call accuracy from Lemon et al. (2017)}
\label{tab:lemon}
\begin{tabular}{|l|c|c|}
\hline
train / test & train accuracy & test accuracy \\ \hline \hline
bAbI/bAbI   & 100 & 100 \\ \hline
bAbI+/bAbI+ & 72  & 53  \\ \hline
bAbI/bAbI+  & 100 & 28  \\ \hline
bAbI+/bAbI  & 67  & 99  \\ \hline
\end{tabular}
\end{table}

More surprising is that results indicate that Seq2seq models perform better at learning the bAbI+ task, achieving a performance of 99.8\% on babi+ to babi+ where Lemon et al. achieved 53\% for their memory network setup. 
Even when not trained on bAbI+ data seq2seq models still achieve a 88\% accuracy, where they achieved 28\$ accuracy with memory networks.


\section{Analysis}

Two questions arise that we try to answer in the following section. 
Why can't the bAbI trained model do the bAbI+ task? and 
How is the model that learned to do the bAbI+ task performing it?
\red{Rephrase first paragraph}

First we look into what are problems the seq2seq model encounters when performing the task without training. To understand what mistakes play a role we will look at some example dialog. 
\red{Introduce quantiative error analysis, maybe type of error classification etc.}

\begin{figure}[h!]
	\centering
\includegraphics[width=.5\textwidth]{images/analysis2.png}
    \caption{Example dialog of babi model on babi+ data}
    \label{fig:babi-babi+}
\end{figure}

A mistake is made for cheap and moderate, based on "in a cheap price range no in a moderate price range". 
Interestingly no mistake is made in "with french cuisine oh no with british cuisine", suggesting that the mistake is not due to the model always picking the first utterance. %, however british is mentioned twice were french is only mentioned once.
This suggests that instead of recognizing the correction and parsing it consistently, the model randomly selects words of the correct type and category. 

The task consists of both conducting dialog and understanding the silver lining of the dialog to predict the API-call. As seen in the example above, normal conversation is conducted well while the mistakes are in grasping the important content from the dialog. 
A split of the error/accuracy over these two subtasks is seen in Table \ref{tab:errorsplit}. This confirms the intuition that grasping the silver lining is the bottle neck that requires training on bAbI+ data. 

\begin{table}[ht!]
\caption{Splitting the results of bAbI trained model on bAbI+ test data}
\label{tab:errorsplit}
\begin{tabular}{|l|c|c|}
\hline& word & sequence \\ \hline
all sequences & 92.5 & 88.1\\
API-calls & 90.2 & 50.8\\
other sequences & 92.8 & 92.8 \\\hline
\end{tabular}
\end{table}

\paragraph{Visualising Attention}
The problem that is mitigated by training on bAbI+ data is thus predicting the correct API-call. 
When predicting API-calls the model uses attention mechanism among other things to direct it's attention. 
Attention is a crucial component, this becomes evident when training a model without attention and sequence accuracies of API-calls approximate zero.

\begin{figure*}[ht]
	\centering
\includegraphics[width=\textwidth]{images/attn11-plus.png}
    \caption{Attention for example of babi+ model on babi+ data}
    \label{fig:babi+-babi+}
\end{figure*}

There are two different patterns of attention in the example sentence: an editing term of "no" and an editing term of "sorry"
%Both a correction with a “no” in the editing term as an example where the editing term is “sorry”.
The bAbI+ trained model only pays attention to the correct form, the alteration, in both cases. 
Suggesting that the plus model in contrast to the previously discussed model, does parse the correction and consistently predicts the correct word.  

It is unclear how the model is doing this. Additional analyses are discussed in the next section that will shed a light on the workings of the model. 
%Conclude the section with the notion that we do not know a lot about how the model is performing its task and that we need inspiration for theories, OR show that the scope of possible theories is really big and introduce theory as a means of tackling this.

%Write short interpretation of results, compare with baselines, do some analysis that is not necessarily linguistic but more common `AI' analysis.
%For instance:\begin{itemize}
%\item sub conclusion about whether models can deal with this or not
%\item API calls are the main issue
%\item Difference attention use between two models?
%\end{itemize}

